Counterfactual (Non-)identifiability of Learned Structural Causal Models

Recent advances in probabilistic generative modeling have motivated learning Structural Causal Models (SCM) from observational datasets using deep conditional generative models, also known as Deep Structural Causal Models (DSCM). If successful, DSCMs can be utilized for causal estimation tasks, e.g., for answering counterfactual queries. In this work, we warn practitioners about non-identifiability of counterfactual inference from observational data, even in the absence of unobserved confounding and assuming known causal structure. We prove counterfactual identifiability of monotonic generation mechanisms with single dimensional exogenous variables. For general generation mechanisms with multi-dimensional exogenous variables, we provide an impossibility result for counterfactual identifiability, motivating the need for parametric assumptions. As a practical approach, we propose a method for estimating worst-case errors of learned DSCMs' counterfactual predictions. The size of this error can be an essential metric for deciding whether or not DSCMs are a viable approach for counterfactual inference in a specific problem setting. In evaluation, our method confirms negligible counterfactual errors for an identifiable SCM from prior work, and also provides informative error bounds on counterfactual errors for a non-identifiable synthetic SCM.

==> clear2023 <==
\begin{thebibliography}{66}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Agarwal et~al.(2020)Agarwal, Shah, and Shen]{si}
Anish Agarwal, Devavrat Shah, and Dennis Shen.
\newblock Synthetic interventions.
\newblock \emph{arXiv preprint arXiv:2006.07691}, 2020.

\bibitem[Alomar et~al.(2022)Alomar, Hamadanian, Nasr-Esfahany, Agarwal,
  Alizadeh, and Shah]{causalsim}
Abdullah Alomar, Pouya Hamadanian, Arash Nasr-Esfahany, Anish Agarwal, Mohammad
  Alizadeh, and Devavrat Shah.
\newblock Causalsim: A causal inference framework for unbiased trace-driven
  simulation.
\newblock 2022.

\bibitem[Arjovsky et~al.(2017)Arjovsky, Chintala, and Bottou]{wgan}
Martin Arjovsky, Soumith Chintala, and L{\'e}on Bottou.
\newblock {W}asserstein generative adversarial networks.
\newblock In Doina Precup and Yee~Whye Teh, editors, \emph{Proceedings of the
  34th International Conference on Machine Learning}, volume~70 of
  \emph{Proceedings of Machine Learning Research}, pages 214--223. PMLR, 06--11
  Aug 2017.
\newblock URL \url{https://proceedings.mlr.press/v70/arjovsky17a.html}.

\bibitem[Bareinboim et~al.(2022)Bareinboim, Correa, Ibeling, and Icard]{pch}
Elias Bareinboim, Juan~D. Correa, Duligur Ibeling, and Thomas Icard.
\newblock \emph{On Pearl’s Hierarchy and the Foundations of Causal
  Inference}, page 507–556.
\newblock Association for Computing Machinery, New York, NY, USA, 1 edition,
  2022.
\newblock ISBN 9781450395861.
\newblock URL \url{https://doi.org/10.1145/3501714.3501743}.

\bibitem[Behrmann et~al.(2019)Behrmann, Duvenaud, and Jacobsen]{i-resnet}
Jens Behrmann, David~Kristjanson Duvenaud, and J{\"o}rn-Henrik Jacobsen.
\newblock Invertible residual networks.
\newblock In \emph{ICML}, 2019.

\bibitem[Blei et~al.(2017)Blei, Kucukelbir, and McAuliffe]{vi1}
David~M Blei, Alp Kucukelbir, and Jon~D McAuliffe.
\newblock Variational inference: A review for statisticians.
\newblock \emph{Journal of the American statistical Association}, 112\penalty0
  (518):\penalty0 859--877, 2017.

\bibitem[Budhathoki et~al.(2022)Budhathoki, Minorics, Bloebaum, and
  Janzing]{root-cause}
Kailash Budhathoki, Lenon Minorics, Patrick Bloebaum, and Dominik Janzing.
\newblock Causal structure-based root cause analysis of outliers.
\newblock In \emph{International Conference on Machine Learning}, pages
  2357--2369. PMLR, 2022.

\bibitem[Correa and Bareinboim(2020{\natexlab{a}})]{soft-calculus}
Juan Correa and Elias Bareinboim.
\newblock A calculus for stochastic interventions: Causal effect identification
  and surrogate experiments.
\newblock In \emph{Proceedings of the AAAI conference on artificial
  intelligence}, volume~34, pages 10093--10100, 2020{\natexlab{a}}.

\bibitem[Correa and Bareinboim(2020{\natexlab{b}})]{soft2}
Juan Correa and Elias Bareinboim.
\newblock General transportability of soft interventions: Completeness results.
\newblock \emph{Advances in Neural Information Processing Systems},
  33:\penalty0 10902--10912, 2020{\natexlab{b}}.

\bibitem[Correa et~al.(2021)Correa, Lee, and Bareinboim]{cf-ident2}
Juan Correa, Sanghack Lee, and Elias Bareinboim.
\newblock Nested counterfactual identification from arbitrary surrogate
  experiments.
\newblock \emph{Advances in Neural Information Processing Systems},
  34:\penalty0 6856--6867, 2021.

\bibitem[Dash et~al.(2022)Dash, Balasubramanian, and
  Sharma]{Dash2022EvaluatingAM}
Saloni Dash, Vineeth~N. Balasubramanian, and Amit Sharma.
\newblock Evaluating and mitigating bias in image classifiers: A causal
  perspective using counterfactuals.
\newblock \emph{2022 IEEE/CVF Winter Conference on Applications of Computer
  Vision (WACV)}, pages 3879--3888, 2022.

\bibitem[Dumoulin et~al.(2016)Dumoulin, Belghazi, Poole, Mastropietro, Lamb,
  Arjovsky, and Courville]{ali}
Vincent Dumoulin, Ishmael Belghazi, Ben Poole, Olivier Mastropietro, Alex Lamb,
  Martin Arjovsky, and Aaron Courville.
\newblock Adversarially learned inference.
\newblock \emph{arXiv preprint arXiv:1606.00704}, 2016.

\bibitem[Durkan et~al.(2019)Durkan, Bekasov, Murray, and
  Papamakarios]{spline-flows}
Conor Durkan, Artur Bekasov, Iain Murray, and George Papamakarios.
\newblock Neural spline flows.
\newblock \emph{Advances in neural information processing systems}, 32, 2019.

\bibitem[Galhotra et~al.(2021)Galhotra, Pradhan, and Salimi]{explainability}
Sainyam Galhotra, Romila Pradhan, and Babak Salimi.
\newblock Explaining black-box algorithms using probabilistic contrastive
  counterfactuals.
\newblock In \emph{Proceedings of the 2021 International Conference on
  Management of Data}, pages 577--590, 2021.

\bibitem[Gan et~al.(2021)Gan, Liang, Dev, Lo, and Delimitrou]{sage}
Yu~Gan, Mingyu Liang, Sundar Dev, David Lo, and Christina Delimitrou.
\newblock Sage: Practical and scalable ml-driven performance debugging in
  microservices.
\newblock In \emph{Proceedings of the 26th ACM International Conference on
  Architectural Support for Programming Languages and Operating Systems},
  ASPLOS '21, page 135–151, New York, NY, USA, 2021. Association for
  Computing Machinery.
\newblock ISBN 9781450383172.
\newblock \doi{10.1145/3445814.3446700}.
\newblock URL \url{https://doi.org/10.1145/3445814.3446700}.

\bibitem[Geffner et~al.(2022)Geffner, Antor{\'a}n, Foster, Gong, Ma, Kıcıman,
  Sharma, Lamb, Kukla, Pawlowski, Allamanis, and Zhang]{deci}
Tomas Geffner, Javier Antor{\'a}n, Adam Foster, Wenbo Gong, Chao Ma, Emre
  Kıcıman, Ajay Sharma, A.~Lamb, Martin Kukla, Nick Pawlowski, Miltiadis
  Allamanis, and Cheng Zhang.
\newblock Deep end-to-end causal inference.
\newblock \emph{ArXiv}, abs/2202.02195, 2022.

\bibitem[Glymour et~al.(2016)Glymour, Pearl, and Jewell]{primer}
Madelyn Glymour, Judea Pearl, and Nicholas~P Jewell.
\newblock \emph{Causal inference in statistics: A primer}.
\newblock John Wiley \& Sons, 2016.

\bibitem[Goodfellow et~al.(2020)Goodfellow, Pouget-Abadie, Mirza, Xu,
  Warde-Farley, Ozair, Courville, and Bengio]{gan}
Ian Goodfellow, Jean Pouget-Abadie, Mehdi Mirza, Bing Xu, David Warde-Farley,
  Sherjil Ozair, Aaron Courville, and Yoshua Bengio.
\newblock Generative adversarial networks.
\newblock \emph{Communications of the ACM}, 63\penalty0 (11):\penalty0
  139--144, 2020.

\bibitem[Gulrajani et~al.(2017)Gulrajani, Ahmed, Arjovsky, Dumoulin, and
  Courville]{gradient-penalty}
Ishaan Gulrajani, Faruk Ahmed, Martin Arjovsky, Vincent Dumoulin, and Aaron~C
  Courville.
\newblock Improved training of wasserstein gans.
\newblock \emph{Advances in neural information processing systems}, 30, 2017.

\bibitem[Ho et~al.(2020)Ho, Jain, and Abbeel]{denoising}
Jonathan Ho, Ajay Jain, and Pieter Abbeel.
\newblock Denoising diffusion probabilistic models.
\newblock \emph{Advances in Neural Information Processing Systems},
  33:\penalty0 6840--6851, 2020.

\bibitem[Hoyer et~al.(2008)Hoyer, Janzing, Mooij, Peters, and
  Sch{\"o}lkopf]{anm2}
Patrik Hoyer, Dominik Janzing, Joris~M Mooij, Jonas Peters, and Bernhard
  Sch{\"o}lkopf.
\newblock Nonlinear causal discovery with additive noise models.
\newblock \emph{Advances in neural information processing systems}, 21, 2008.

\bibitem[Huang et~al.(2018)Huang, Krueger, Lacoste, and Courville]{flow4}
Chin-Wei Huang, David Krueger, Alexandre Lacoste, and Aaron Courville.
\newblock Neural autoregressive flows.
\newblock In \emph{International Conference on Machine Learning}, pages
  2078--2087. PMLR, 2018.

\bibitem[Hyv{\"a}rinen and Pajunen(1999)]{hyvarinen1999nonlinear}
Aapo Hyv{\"a}rinen and Petteri Pajunen.
\newblock Nonlinear independent component analysis: Existence and uniqueness
  results.
\newblock \emph{Neural networks}, 12\penalty0 (3):\penalty0 429--439, 1999.

\bibitem[Jaber et~al.(2020)Jaber, Kocaoglu, Shanmugam, and Bareinboim]{soft3}
Amin Jaber, Murat Kocaoglu, Karthikeyan Shanmugam, and Elias Bareinboim.
\newblock Causal discovery from soft interventions with unknown targets:
  Characterization and learning.
\newblock \emph{Advances in neural information processing systems},
  33:\penalty0 9551--9561, 2020.

\bibitem[Jaiswal et~al.(2018)Jaiswal, AbdAlmageed, Wu, and
  Natarajan]{bidirectional-gan}
Ayush Jaiswal, Wael AbdAlmageed, Yue Wu, and Premkumar Natarajan.
\newblock Bidirectional conditional generative adversarial networks.
\newblock In \emph{Asian Conference on Computer Vision}, pages 216--232.
  Springer, 2018.

\bibitem[Jordan et~al.(1999)Jordan, Ghahramani, Jaakkola, and Saul]{vi2}
Michael~I Jordan, Zoubin Ghahramani, Tommi~S Jaakkola, and Lawrence~K Saul.
\newblock An introduction to variational methods for graphical models.
\newblock \emph{Machine learning}, 37\penalty0 (2):\penalty0 183--233, 1999.

\bibitem[Khemakhem et~al.(2021)Khemakhem, Monti, Leech, and
  Hyv{\"a}rinen]{Khemakhem2021CausalAF}
Ilyes Khemakhem, Ricardo~Pio Monti, Robert Leech, and Aapo Hyv{\"a}rinen.
\newblock Causal autoregressive flows.
\newblock \emph{ArXiv}, abs/2011.02268, 2021.

\bibitem[Kingma and Welling(2014)]{vae}
Diederik~P. Kingma and Max Welling.
\newblock Auto-encoding variational bayes.
\newblock In Yoshua Bengio and Yann LeCun, editors, \emph{2nd International
  Conference on Learning Representations, {ICLR} 2014, Banff, AB, Canada, April
  14-16, 2014, Conference Track Proceedings}, 2014.
\newblock URL \url{http://arxiv.org/abs/1312.6114}.

\bibitem[Kingma et~al.(2016)Kingma, Salimans, Jozefowicz, Chen, Sutskever, and
  Welling]{flow3}
Durk~P Kingma, Tim Salimans, Rafal Jozefowicz, Xi~Chen, Ilya Sutskever, and Max
  Welling.
\newblock Improved variational inference with inverse autoregressive flow.
\newblock \emph{Advances in neural information processing systems}, 29, 2016.

\bibitem[Kobyzev et~al.(2019)Kobyzev, Prince, and Brubaker]{NF2}
Ivan Kobyzev, Simon Prince, and Marcus~A. Brubaker.
\newblock Normalizing flows: Introduction and ideas.
\newblock \emph{ArXiv}, abs/1908.09257, 2019.

\bibitem[Kusner et~al.(2017)Kusner, Loftus, Russell, and Silva]{fairness}
Matt~J Kusner, Joshua Loftus, Chris Russell, and Ricardo Silva.
\newblock Counterfactual fairness.
\newblock \emph{Advances in neural information processing systems}, 30, 2017.

\bibitem[Lagnado et~al.(2013)Lagnado, Gerstenberg, and Zultan]{legal}
David~A Lagnado, Tobias Gerstenberg, and Ro'i Zultan.
\newblock Causal responsibility and counterfactuals.
\newblock \emph{Cognitive science}, 37\penalty0 (6):\penalty0 1036--1073, 2013.

\bibitem[Lang(2005)]{monotone2}
Bernhard Lang.
\newblock Monotonic multi-layer perceptron networks as universal approximators.
\newblock In \emph{International conference on artificial neural networks},
  pages 31--37. Springer, 2005.

\bibitem[Lasserre(2001)]{polynomial1}
Jean~B Lasserre.
\newblock Global optimization with polynomials and the problem of moments.
\newblock \emph{SIAM Journal on optimization}, 11\penalty0 (3):\penalty0
  796--817, 2001.

\bibitem[Li(2021)]{ads}
Ang Li.
\newblock \emph{Unit selection based on counterfactual logic}.
\newblock University of California, Los Angeles, 2021.

\bibitem[Locatello et~al.(2019)Locatello, Bauer, Lucic, Raetsch, Gelly,
  Sch{\"o}lkopf, and Bachem]{locatello2019challenging}
Francesco Locatello, Stefan Bauer, Mario Lucic, Gunnar Raetsch, Sylvain Gelly,
  Bernhard Sch{\"o}lkopf, and Olivier Bachem.
\newblock Challenging common assumptions in the unsupervised learning of
  disentangled representations.
\newblock In \emph{international conference on machine learning}, pages
  4114--4124. PMLR, 2019.

\bibitem[Lorberbom et~al.(2021)Lorberbom, Johnson, Maddison, Tarlow, and
  Hazan]{disc3}
Guy Lorberbom, Daniel~D Johnson, Chris~J Maddison, Daniel Tarlow, and Tamir
  Hazan.
\newblock Learning generalized gumbel-max causal mechanisms.
\newblock \emph{Advances in Neural Information Processing Systems},
  34:\penalty0 26792--26803, 2021.

\bibitem[Lu et~al.(2020)Lu, Huang, Wang, Hern{\'a}ndez-Lobato, Zhang, and
  Sch{\"o}lkopf]{rlcf}
Chaochao Lu, Biwei Huang, Ke~Wang, Jos{\'e}~Miguel Hern{\'a}ndez-Lobato, Kun
  Zhang, and Bernhard Sch{\"o}lkopf.
\newblock Sample-efficient reinforcement learning via counterfactual-based data
  augmentation.
\newblock \emph{arXiv preprint arXiv:2012.09092}, 2020.

\bibitem[Mesnard et~al.(2021)Mesnard, Weber, Viola, Thakoor, Saade,
  Harutyunyan, Dabney, Stepleton, Heess, Guez, et~al.]{credit}
Thomas Mesnard, Theophane Weber, Fabio Viola, Shantanu Thakoor, Alaa Saade,
  Anna Harutyunyan, Will Dabney, Thomas~S Stepleton, Nicolas Heess, Arthur
  Guez, et~al.
\newblock Counterfactual credit assignment in model-free reinforcement
  learning.
\newblock In \emph{International Conference on Machine Learning}, pages
  7654--7664. PMLR, 2021.

\bibitem[Miyato et~al.(2018)Miyato, Kataoka, Koyama, and Yoshida]{spec-norm}
Takeru Miyato, Toshiki Kataoka, Masanori Koyama, and Yuichi Yoshida.
\newblock Spectral normalization for generative adversarial networks.
\newblock In \emph{International Conference on Learning Representations}, 2018.

\bibitem[Mohamed and Lakshminarayanan(2016)]{implicit}
Shakir Mohamed and Balaji Lakshminarayanan.
\newblock Learning in implicit generative models.
\newblock \emph{ArXiv}, abs/1610.03483, 2016.

\bibitem[Oberst and Sontag(2019)]{disc2}
Michael Oberst and David Sontag.
\newblock Counterfactual off-policy evaluation with gumbel-max structural
  causal models.
\newblock In \emph{International Conference on Machine Learning}, pages
  4881--4890. PMLR, 2019.

\bibitem[Papamakarios et~al.(2021)Papamakarios, Nalisnick, Rezende, Mohamed,
  and Lakshminarayanan]{NF1}
George Papamakarios, Eric~T. Nalisnick, Danilo~Jimenez Rezende, Shakir Mohamed,
  and Balaji Lakshminarayanan.
\newblock Normalizing flows for probabilistic modeling and inference.
\newblock \emph{J. Mach. Learn. Res.}, 22:\penalty0 57:1--57:64, 2021.

\bibitem[Parrilo(2003)]{polynomial2}
Pablo~A Parrilo.
\newblock Semidefinite programming relaxations for semialgebraic problems.
\newblock \emph{Mathematical programming}, 96\penalty0 (2):\penalty0 293--320,
  2003.

\bibitem[Pawlowski et~al.(2020)Pawlowski, Coelho~de Castro, and
  Glocker]{Pawlowski2020DeepSC}
Nick Pawlowski, Daniel Coelho~de Castro, and Ben Glocker.
\newblock Deep structural causal models for tractable counterfactual inference.
\newblock \emph{Advances in Neural Information Processing Systems},
  33:\penalty0 857--869, 2020.

\bibitem[Pearl(2009)]{causality-book}
Judea Pearl.
\newblock \emph{Causality}.
\newblock Cambridge university press, 2009.

\bibitem[Pearl and Mackenzie(2018)]{why}
Judea Pearl and Dana Mackenzie.
\newblock \emph{The book of why: the new science of cause and effect}.
\newblock Basic books, 2018.

\bibitem[Peters et~al.(2010)Peters, Janzing, and Sch{\"o}lkopf]{anm1}
Jonas Peters, Dominik Janzing, and Bernhard Sch{\"o}lkopf.
\newblock Identifying cause and effect on discrete data using additive noise
  models.
\newblock In \emph{Proceedings of the thirteenth international conference on
  artificial intelligence and statistics}, pages 597--604. JMLR Workshop and
  Conference Proceedings, 2010.

\bibitem[Peters et~al.(2014)Peters, Mooij, Janzing, and Sch{\"o}lkopf]{anm3}
Jonas Peters, Joris~M Mooij, Dominik Janzing, and Bernhard Sch{\"o}lkopf.
\newblock Causal discovery with continuous additive noise models.
\newblock 2014.

\bibitem[Peters et~al.(2017)Peters, Janzing, and Sch{\"o}lkopf]{elements}
Jonas Peters, Dominik Janzing, and Bernhard Sch{\"o}lkopf.
\newblock \emph{Elements of causal inference: foundations and learning
  algorithms}.
\newblock 2017.

\bibitem[Rezende and Mohamed(2015)]{flow2}
Danilo Rezende and Shakir Mohamed.
\newblock Variational inference with normalizing flows.
\newblock In \emph{International conference on machine learning}, pages
  1530--1538. PMLR, 2015.

\bibitem[Richens et~al.(2020)Richens, Lee, and Johri]{medicine}
Jonathan~G Richens, Ciar{\'a}n~M Lee, and Saurabh Johri.
\newblock Improving the accuracy of medical diagnosis with causal machine
  learning.
\newblock \emph{Nature communications}, 11\penalty0 (1):\penalty0 1--9, 2020.

\bibitem[Richens et~al.(2022)Richens, Beard, and Thompson]{harm}
Jonathan~G. Richens, Rory Beard, and Daniel~H. Thompson.
\newblock Counterfactual harm.
\newblock 2022.

\bibitem[Sanchez and Tsaftaris(2022)]{Sanchez2022DiffusionCM}
Pedro Sanchez and Sotirios~A. Tsaftaris.
\newblock Diffusion causal models for counterfactual estimation.
\newblock In \emph{CLeaR}, 2022.

\bibitem[Sharma et~al.(2021)Sharma, Syrgkanis, Zhang, and K{\i}c{\i}man]{dowhy}
Amit Sharma, Vasilis Syrgkanis, Cheng Zhang, and Emre K{\i}c{\i}man.
\newblock Dowhy: Addressing challenges in expressing and validating causal
  assumptions.
\newblock \emph{arXiv preprint arXiv:2108.13518}, 2021.

\bibitem[Shpitser and Pearl(2008)]{shpitser2008complete}
Ilya Shpitser and Judea Pearl.
\newblock Complete identification methods for the causal hierarchy.
\newblock \emph{Journal of Machine Learning Research}, 9:\penalty0 1941--1979,
  2008.

\bibitem[Shpitser and Pearl(2012)]{cf-ident1}
Ilya Shpitser and Judea Pearl.
\newblock What counterfactuals can be tested.
\newblock \emph{arXiv preprint arXiv:1206.5294}, 2012.

\bibitem[Song and Ermon(2019)]{score}
Yang Song and Stefano Ermon.
\newblock Generative modeling by estimating gradients of the data distribution.
\newblock \emph{Advances in Neural Information Processing Systems}, 32, 2019.

\bibitem[Squires and Uhler(2022)]{discovery1}
Chandler Squires and Caroline Uhler.
\newblock Causal structure learning: a combinatorial perspective.
\newblock \emph{arXiv preprint arXiv:2206.01152}, 2022.

\bibitem[Sutton and Barto(2018)]{rl}
Richard~S Sutton and Andrew~G Barto.
\newblock \emph{Reinforcement learning: An introduction}.
\newblock MIT press, 2018.

\bibitem[Vlontzos et~al.(2022)Vlontzos, Kainz, and Lee]{disc1}
Athanasios Vlontzos, Bernhard Kainz, and Ciar{\'a}n Lee.
\newblock Estimating categorical counterfactuals via deep twin networks.
\newblock 2022.

\bibitem[Witty et~al.(2021)Witty, Jensen, and Mansinghka]{emp2}
Sam Witty, David Jensen, and Vikash Mansinghka.
\newblock A simulation-based test of identifiability for bayesian causal
  inference.
\newblock \emph{arXiv preprint arXiv:2102.11761}, 2021.

\bibitem[Xia et~al.(2021)Xia, Lee, Bengio, and Bareinboim]{emp1}
Kevin Xia, Kai-Zhan Lee, Yoshua Bengio, and Elias Bareinboim.
\newblock The causal-neural connection: Expressiveness, learnability, and
  inference.
\newblock \emph{Advances in Neural Information Processing Systems},
  34:\penalty0 10823--10836, 2021.

\bibitem[Zhang et~al.(2018)Zhang, B{\"u}tepage, Kjellstr{\"o}m, and Mandt]{vi3}
Cheng Zhang, Judith B{\"u}tepage, Hedvig Kjellstr{\"o}m, and Stephan Mandt.
\newblock Advances in variational inference.
\newblock \emph{IEEE transactions on pattern analysis and machine
  intelligence}, 41\penalty0 (8):\penalty0 2008--2026, 2018.

\bibitem[Zhang and Zhang(1999)]{monotone1}
Hong Zhang and Zhen Zhang.
\newblock Feedforward networks with monotone constraints.
\newblock In \emph{IJCNN'99. International Joint Conference on Neural Networks.
  Proceedings (Cat. No.99CH36339)}, volume~3, pages 1820--1823 vol.3, 1999.
\newblock \doi{10.1109/IJCNN.1999.832655}.

\bibitem[Zhang et~al.(2022)Zhang, Tian, and Bareinboim]{partial}
Junzhe Zhang, Jin Tian, and Elias Bareinboim.
\newblock Partial counterfactual identification from observational and
  experimental data.
\newblock In \emph{International Conference on Machine Learning}, pages
  26548--26558. PMLR, 2022.

\end{thebibliography}

